Efficient Algorithms for Earliest and Fastest Paths in Public Transport Networks

Public transport administrators rely on efficient algorithms for various problems that arise in public transport networks. In particular, our study focused on designing linear-time algorithms for two fundamental path problems: the earliest arrival time (\textsc{eat}) and the fastest path duration (\textsc{fpd}) on public transportation data. We conduct a comparative analysis with state-of-the-art algorithms. The results are quite promising, indicating substantial efficiency improvements. Specifically, the fastest path problem shows a remarkable 34-fold speedup, while the earliest arrival time problem exhibits an even more impressive 183-fold speedup. These findings highlight the effectiveness of our algorithms to solve \textsc{eat} and \textsc{fpd} problems in public transport, and eventually help public administrators to enrich the urban transport experience.

==> TexFiles/AlgoCorrectness.tex <==
\section{Algorithms and Correctness}
\subsection{Earliest Arrival Time Problem}
In this subsection, we introduce our algorithm for calculating the earliest arrival time from a source vertex $s$ to all other vertices in $G$, for a given ready time $dt$.

\begin{algorithm2e}[H]
\caption{Earliest Arrival Time in Temporal Graph}
\label{algoEarliestPathVersion1}
\SetAlgoLined
\KwIn{A source vertex $s$, ready time at source $dt$ and edge scan dependency graph $\Tilde{G}$ of a temporal graph $G$.}
\KwOut{ For each vertex $z$ in $G$, the earliest arrival time from $s$ to $z$.}

\lFor{each vertex $z$ $\in$ $G$ $\setminus$ $s$}{ $eat[z]$ = $\infty$ } $eat[s] = dt$ \;
\For{each node $x \in  \Tilde{G}$ such that $\leftvertex(x)==src$ and $\dep(x) \geq dt$ }
{
    \For{each path \textsc{p} from $x$ to a node $y$ in $\Tilde{G}$}
    {
          $\eat[\rightvertex(y)] = \min\{ \eat[\rightvertex(y)], \arr(y) \}$ \label{algoLineEATUpdate} \;
    }

}
\end{algorithm2e}

\begin{theorem}
    Given an ESDG $\Tilde{G}$ of a temporal graph $G$, source vertex $s$ in $G$ and a ready time $dt$,  Algorithm \ref{algoEarliestPathVersion1} correctly computes the earliest arrival time from $s$ to every vertex in $G$.
\end{theorem}

\begin{proof}
    Let $z$ be a vertex in $G$ such that $z\neq s$. We now prove that, after all the iterations of Algorithm~\ref{algoEarliestPathVersion1} are over, $\eat[z]$ is equal to the earliest arrival time from $s$ to $z$. 
    In Algorithm~\ref{algoEarliestPathVersion1}, for every node $x$ in  $\Tilde{G}$ such that $\leftvertex(x)=s$ and $\dep(x)\geq dt$, we traverse from $x$, go through all the paths to find all reachable nodes in $\Tilde{G}$.
    The arrival times of all these paths are considered and stored the minimum one in $\eat[z]$ in Line~\ref{algoLineEATUpdate}.
    Also, these paths in $\Tilde{G}$ precisely correspond to those useful dominating paths from $s$ to $z$ in $G$ whose departure time is at least $dt$, due to Lemma~\ref{lemmaESDGTransformation1}.
    From Corollary~\ref{corollaryEPisUseful}, it is sufficient to consider useful dominating paths from $s$ to $z$ that depart at time at least $dt$, to obtain an earliest arrival path from $s$ to $z$,  for the given departure time $dt$. Thus the theorem holds true.  
\end{proof}

\subsection{Fastest Path duration}
In this sub-section, we proposed an efficient  algorithm for computing the fastest path duration from the source vertex to the rest of the vertices present in the graph $G$ based on the given source vertex.

\begin{algorithm2e}[H]
\caption{1  - All Fastest Path Algorithm using ESDG}
\label{algoFastestPathVersion1}
\SetAlgoLined
\KwIn{A source vertex $s$, and an edge scan dependency graph $\Tilde{G}$ of a temporal graph $G$}
\KwOut{For each vertex $z$ in $G$, the  fastest duration from $s$ to $z$.}

\lFor{each vertex $z$ in ${G}$ $\setminus$ $s$}{ $\journey[z] = \infty$} \label{startinitV1}
$\journey[s]=0$ \;
\For{each node $x$ in $\Tilde{G}$, such that $\leftvertex(x)=s$}
{
    \For{each each path \textsc{p} from $x$ to a node $y$ in $\Tilde{G}$}
    {
          $\journey[\rightvertex(y)] = \min\{ \journey[\rightvertex(y)], \arr(y)-\dep(x) \}$ \label{algoLineJourneyUpdate} \;
    } 
} \label{LineAlgoV1Phaseend}
\end{algorithm2e}


\begin{theorem}
    Algorithm \ref{algoFastestPathVersion1} correctly computes the fastest path duration from a source vertex $src$ to every vertex in $G$.
\end{theorem}

\begin{proof}
Let $z$ be a vertex in $G$ such that $z\neq s$. We now show that, after all the iterations of Algorithm~\ref{algoFastestPathVersion1} are over, $\journey[z]$ is equal to the journey time of a fastest path from $s$ to $z$. 
In Algorithm~\ref{algoFastestPathVersion1}, for every node $x$ in  $\Tilde{G}$ such that $\leftvertex(x)=s$, we traverse from $x$, go through all the paths to find all  reachable nodes in $\Tilde{G}$.
%The key step in the algorithm is to traverse through all the paths that originate at x and find all the all reachable nodes in $\Tilde{G}$
%find all paths from $x$ to the all reachable nodes in $\Tilde{G}$, where $x \in \delta_{out}(s)$. 
Out of all these paths, let us observe all those paths that end at $y$, such that  $\rightvertex(y)=z$.
%  $y\in \delta_{in}(z)$.
The journey times of all these paths are considered and stored the minimum one in $\journey[z]$ in Line~\ref{algoLineJourneyUpdate}.
Also, these paths in $\Tilde{G}$ precisely correspond to the useful dominating paths from $s$ to $z$ in $G$ due to Lemma~\ref{lemmaESDGTransformation1}.
%Since every fastest path is a useful dominating path, it is sufficient to consider all useful dominating paths.
%Processing all useful dominating paths from $s$ to $z$ in $G$ is sufficient to obtain a fastest path from s t z, because of Leamma~\ref{}.
%For every fastest path p from s to z, there exist a useful dominating path q from s to z, such that journey(p) = journey(q)
From Corollary~\ref{corollaryFPisUseful}, it is sufficient to consider useful dominating paths from $s$ to $z$ to obtain a fastest path from $s$ to $z$.
Thus the theorem holds true.
\end{proof}


% To prove that Algorithm \ref{FPDAlgo} correctly computes the fastest path duration for any vertex $v \in G$, we need to show two cases:

% Case 1: If a fastest path from $src$ to $v$ exists in $G$:
% In this case, there exists a path from the source vertex $src$ to vertex $v$ in the graph $G$ that has the minimum duration. Algorithm \ref{FPDAlgo} guarantees to compute the correct fastest path duration for $v$ as it iteratively updates the $\journey$ values based on the minimum duration among all incoming edges. By the end of the algorithm, $\journey[v]$ will store the duration of the fastest path from $src$ to $v$.

% Case 2: If a fastest path from $src$ to $v$ does not exist in $G$:
% In this case, there is no path from the source vertex $src$ to vertex $v$ in the graph $G$. In Algorithm \ref{FPDAlgo}, the initial value of $\journey[v]$ is set to $\infty$ for all vertices. Since there is no path from $src$ to $v$, the algorithm will not encounter any incoming edges for $v$, and its $\journey[v]$ value will remain $\infty$ after the algorithm's execution.

% Therefore, Algorithm \ref{FPDAlgo} correctly computes the fastest path duration for any vertex $v \in G$ if a fastest path from $src$ to $v$ exists in $G$. Otherwise, it correctly assigns $\journey[v]$ as $\infty$.
% \end{proof}

==> TexFiles/AlgoOptimizations.tex <==
\section{Algorithms and Optimizations}
\subsection{Earliest Arrival Time Problem}

\begin{algorithm2e}[H]
\caption{Earliest Arrival Time in Temporal Graph}
\SetAlgoLined
\KwIn{A source vertex $s$, ready time at source $dt$ and edge scan dependency graph $\Tilde{G}$ of a temporal graph $G$.}
\KwOut{ For each vertex $z$ in $G$, the earliest arrival time from $s$ to $z$.}

\lFor{each vertex $z$ $\in$ $G$ $\setminus$ $s$}{ $eat[z]$ = $\infty$ } $eat[src] = 0$ \; \label{LinestartinitEAT}
\lFor{each node $x=(u,v,t, \lambda) \in  \Tilde{G}$}{ $visited[x]=false$ }                  \label{LinestendinitEAT}
\For{each node $x=(u,v,t, \lambda) \in  \Tilde{G}$ such that $x.u==src$ and $x.t \geq dt$ }
{
    $q.insert(x)$ ;   $visited[x] = true$  \;
    \While{$(|q|\geq 1)$}
    {
        $x = q.pop()$ \;
        $eat[x.v] = min(eat[x.v],x.t+ x.\lambda)$ \;   \label{algoLineEATUpdate}
        \lFor{\textbf{each} neighbor $y$ of $x$ in $\Tilde{G}$ such that $visited[y]== false$ }{ $q.insert(y)$ } 
    }     
}
\end{algorithm2e}

\noindent \textbf{optimization-1}:
%Let y be a reachable node from x_i and x_j such that \leftvertex(x_i)=\leftvertex(x_j)=s,  \dep(x_i)\geq rt, and \dep(x_j) \geq rt. P_i, P_j
The earliest arrival times of both $P_i$ and $P_j$ are same because both paths are arriving at $\arr(y)$. Hence, we can avoid processing a node that was visited earlier. 

\noindent \textbf{optimization-2}:
%Let y be an outgoing neighbour of x_i.
If $xi.t + xi.\lambda \geq eat[xi.v]$, then we can skip inserting the  outgoing neighbours of $x_i$ in the queue because they would have been inserted in the previous iterations.
Let $x_j$ be the node such that $eat[v]$ was updated when $x_j$ is processed.
Then, $y$ would have been inserted in the queue when $x_j$ was processed.







Given a source vertex $s$, departure time at the source $dt$, and an ESDG graph $\Tilde{G}$, the algorithm initializes the earliest arrival time $\eat[z]$ for each vertex $z \in V$. The earliest arrival time represents the minimum time to reach vertex $z$ from the source vertex $s$. During the initialization phase (lines~\ref{LinestartinitEAT}-\ref{LinestendinitEAT}), all vertices (except the source) are set to have an earliest arrival time of $\infty$, while the source vertex is set to $dt$. The queue $Q$ is also initialized with valid connections where $u=src$ and the departure time at the source vertex is greater than or equal to $t$.

After the initialization, the algorithm proceeds to process connections by dequeuing them one by one and performing relaxation. If a connection is successfully relaxed, its neighboring vertices are added to the queue. These two steps are repeated until the queue becomes empty.
\subsection{Efficient Algorithm for Fastest Path Duration}

%For each node $x \in \Tilde{G}$, such that $\leftvertex(x)=s$, we process t
%The process of identifying all the reachable nodes 
%For every node $x$ in $G'$ such that $leftvertex(x)=s$, the process of identifying all the reachable nodes from $x$ and processing them need not be independent. 

\textcolor{blue}{connecting sentence}

Let $x_i$ and $x_j$ be two nodes in $\tilde{G}$ such that $\leftvertex(x_i)= \leftvertex(x_j)=s$, and are selected in the outer loop iterations $i$ and $j$, respectively, in Line~\ref{df} of Algorithm~\ref{sdf} . Let $y$ be a node that is reachable from $x_i$ and $x_j$. Further, let $P_i$ denote a path from $x_i$ to $y$, $P_j$ denote a path from $x_j$ to $y$. If $\dep(x_j) \leq \dep(x_i)$, then $\journey(P_j) \geq \journey(P_i)$, because $\arr(P_i) = \arr(P_j)$. This observation leads to the following key optimization. 
A node $y$  that has been processed in the $i^{th}$ iteration of the outer loop need not be processed in the  $j^{th}$ iteration of the outer loop,
if $\dep(x_j) \leq \dep(x_i)$, because the journey from $s$ to $\rightvertex(y)$ does not decrease. 
For gaining the benefits from this optimization, we perform traversals from all the nodes in the edge scan dependency graph, whose left vertex is the source vertex, in the decreasing order based on their departure time, and avoid processing nodes that were processed earlier. 

 %   Let $x$ be a node in $\tilde{G}$ that was visited in the $j^{th}$ iteration, where $1 \leq j \leq i-1$.  Let $P'$ be the corresponding path. Furthermore, let $P$ be a path from $s$ to $t_i$ via $x$, with $x$ ending at $v_i$. We can observe that $\journey(P) \geq \journey[v_i]$. This is because both $P$ and $P'$ have the same arrival time, denoted by $arrivalTime(P') = arrivalTime(P)$. Additionally, we have $departureTime(P) < departureTime(P')$ and $\journey(P') \geq \journey[v_i]$. Therefore, extending the traversal by considering $x$ and the path $P$ does not decrease the journey time required to reach $v_i$. As a result, we can early terminate and prune the visited nodes in the subsequent iterations, knowing that the current path $P'$ already provides a faster journey time to reach $v_i$.

\begin{algorithm2e}[H]
\caption{1  - All Fastest Path Algorithm using ESDG}
\label{algoFastestPathVersion2}
  \SetAlgoLined
\KwIn{A source vertex $src$, and an edge scan dependency graph $\Tilde{G}$ of a temporal graph $G$}
\KwOut{For each vertex $x$ in $G$, the  fastest duration from $src$ to $x$.}

\lFor{each vertex $v$ in ${G}$ $\setminus$ $src$}{ $\journey[v] = \infty$} \label{startinitFPD}
$\journey[src]=0$
\lFor{each node $x=(u,v,t,\lambda)$ in $\Tilde{G}$}{ $s[x] = - 1 $ }  \label{endinitFPD}
\For{each node $x=(u,v,t,\lambda)$ in $\Tilde{G}$ such that $x.u==src$ and decreasing order of $x.t$}
{
    $q.insert(x)$ \label{LineAlgoInit_v1};
    $s[x] = x.t$ \;
    \While{$(|q|\geq 1)$}
    {
        $x = q.pop()$ \;
        $\journey[x.v] = min(\journey[x.v],x.t+ x.\lambda - s[x])$ \;
        \lFor{each neighbor $y$ of $x$  in $\Tilde{G}$ such that $s[y] == -1 $} { $s[y] = s[x]$; $q.insert(y)$ }
    }
}
\end{algorithm2e}

%In this algorithm \ref{algoFastestPathVersion2}, we utilize a single queue to process connections, eliminating the need for maintaining a list of tuples at each vertex. By employing a pruning technique, we process only a minimal number of connections.
We now provide the detailed description of our algorithm to solve \textsc{fastest path duration}, whose pseudo-code is given in Algorithm~\ref{df}.
For each vertex $z$ in $G$, the variable $\journey[z]$ stores the journey time, representing the fastest path duration from the source vertex $s$ to $z$.
For each node $x$ in $\Tilde{G}$, we use $s[x]$ to store the starting time of a journey that departs as late as possible from $s$ and  reaches node $x$.
We use $q$ to denote the queue data structure, which helps to perform breadth first kind of traversal.
During the initialization phase (lines~\ref{startinitFPD}-\ref{endinitFPD}), we set the fastest path duration of all vertices, except the source vertex, as $\infty$. The fastest path duration of the source vertex is set to $0$.
We now go through each node $x$  in $\Tilde{G}$ such that $x.u==src$ in decreasing order based on the departure time of the nodes, and perform breadth first search kind of traversal to identify reachable nodes from $x$ as follows.
We insert $x$ in the queue $q$, and initialize $s[x]$ with its departure time. 
As long as the queue is not empty, we extract a node $x$ from the queue and update  $\journey[x.v]$ if $t+\lambda-s[x])$ is lesser than $\journey[x.v]$. Afterwards, we insert each neighbor $y$ of $x$ into the queue $q$ and update $s[y]$ with the maximum value between $s[y]$ and $s[x]$. This algorithm only processes the nodes (connections) that are inserted into the queue. 
\textcolor{blue}{By checking if the respective connection starting time is not set (i.e., -1), we optimize the algorithm to reduce unnecessary connection processing, thereby lowering the processing time.} Finally, $\journey[v]$ holds the fastest path duration from $src$ to any vertex $v$ due to Theorem~\ref{sf}..


